Cucheb: A GPU implementation of the filtered Lanczos procedure

This paper describes the software package Cucheb, a GPU implementation of the filtered Lanczos procedure for the solution of large sparse symmetric eigenvalue problems. The filtered Lanczos procedure uses a carefully chosen polynomial spectral transformation to accelerate convergence of the Lanczos method when computing eigenvalues within a desired interval. This method has proven particularly effective for eigenvalue problems that arise in electronic structure calculations and density functional theory. We compare our implementation against an equivalent CPU implementation and show that using the GPU can reduce the computation time by more than a factor of 10.

==> engineering_table.tex <==
\begin{tabular}{lccccccc}
\hline
\multirow{2}{*}{Matrix} & \multirow{2}{*}{fraction} & \multirow{2}{*}{eigs} & \multirow{2}{*}{$m$} & \multirow{2}{*}{iters} & \multirow{2}{*}{MV} & \multirow{2}{*}{time} & \multirow{2}{*}{residual} \\
 & & & & & & & \\\hline
\hline
\multirow{2}{*}{\texttt{fe\_ocean}} & \multirow{2}{*}{$\phantom{0}2$\%} & \multirow{2}{*}{$217$} & $47$ & $\phantom{0,{}}480$ & $22,560$ & $\phantom{0}19$ & $1.3e{-12}$ \\
 & & & $\phantom{0}1$ & $4,200$ & $\phantom{0}4,200$ & $803$ & $2.9e{-14}$ \\\hline
\multirow{2}{*}{\texttt{144}} & \multirow{2}{*}{$\phantom{0}4$\%} & \multirow{2}{*}{$195$} & $33$ & $\phantom{0,{}}450$ & $14,850$ & $\phantom{0}19$ & $1.7e{-12}$ \\
 & & & $\phantom{0}1$ & $2,700$ & $\phantom{0}2,700$ & $252$ & $4.1e{-13}$ \\\hline
\multirow{2}{*}{\texttt{m14b}} & \multirow{2}{*}{$\phantom{0}3$\%} & \multirow{2}{*}{$235$} & $38$ & $\phantom{0,{}}510$ & $19,380$ & $\phantom{0}37$ & $1.3e{-12}$ \\
 & & & $\phantom{0}1$ & $3,600$ & $\phantom{0}3,600$ & $833$ & $3.2e{-14}$ \\\hline
\multirow{2}{*}{\texttt{auto}} & \multirow{2}{*}{$\phantom{0}4$\%} & \multirow{2}{*}{$172$} & $33$ & $\phantom{0,{}}390$ & $12,870$ & $\phantom{0}56$ & $1.8e{-11}$ \\
 & & & $\phantom{0}1$ & $2,700$ & $\phantom{0}2,700$ & $961$ & $3.5e{-14}$ \\\hline
\end{tabular}

==> engineering_table2.tex <==
\begin{tabular}{lcccc}
\hline
\multirow{2}{*}{Matrix} & \multirow{2}{*}{$m$} & \multirow{2}{*}{iters} & \multirow{2}{*}{ORTH}& \multirow{2}{*}{MV} \\
 & & & & \\\hline
\hline
\multirow{2}{*}{\texttt{fe\_ocean}} & $47$ & $\phantom{0,{}}480$ & $29$\% & $25$\%\\
  & $\phantom{0}1$ & $4,200$ & $35$\% & ${}<\!\! 1$\%\\\hline
\multirow{2}{*}{\texttt{144}} & $33$ & $\phantom{0,{}}450$ & $27$\% & $43$\%\\
  & $\phantom{0}1$ & $2,700$ & $47$\% & $\phantom{0}1$\%\\\hline
\multirow{2}{*}{\texttt{m14b}} & $38$ & $\phantom{0,{}}510$ & $25$\% & $48$\%\\
  & $\phantom{0}1$ & $3,600$ & $56$\% & ${}<\!\! 1$\%\\\hline
\multirow{2}{*}{\texttt{auto}} & $33$ & $\phantom{0,{}}390$ & $23$\% & $56$\%\\
  & $\phantom{0}1$ & $2,700$ & $73$\% & $\phantom{0}1$\%\\\hline
\end{tabular}

==> graph_table.tex <==
\begin{tabular}{lccccccc}
\hline
\multirow{2}{*}{Matrix} & \multirow{2}{*}{fraction} & \multirow{2}{*}{eigs} & \multirow{2}{*}{$m$} & \multirow{2}{*}{iters} & \multirow{2}{*}{MV} & \multirow{2}{*}{time} & \multirow{2}{*}{residual} \\
 & & & & & & & \\\hline
\hline
\multirow{2}{*}{\texttt{caidaRouterLevel}} & \multirow{2}{*}{$42$\%} & \multirow{2}{*}{$137$} & $10$ & $570$ & $5,700$ & $\phantom{0}21$ & $1.2e{-12}$ \\
 & & & $\phantom{0}1$ & $780$ & $\phantom{0,{}}780$ & $\phantom{0}41$ & $1.8e{-14}$ \\\hline
\multirow{2}{*}{\texttt{mn2010}} & \multirow{2}{*}{$42$\%} & \multirow{2}{*}{$\phantom{0}79$} & $10$ & $360$ & $3,600$ & $\phantom{0}13$ & $3.0e{-13}$ \\
 & & & $\phantom{0}1$ & $510$ & $\phantom{0,{}}510$ & $\phantom{0}21$ & $1.9e{-14}$ \\\hline
\multirow{2}{*}{\texttt{coPapersDBLP}} & \multirow{2}{*}{$50$\%} & \multirow{2}{*}{$134$} & $\phantom{0}9$ & $360$ & $3,240$ & $\phantom{0}44$ & $2.1e{-11}$ \\
 & & & $\phantom{0}1$ & $630$ & $\phantom{0,{}}630$ & $\phantom{0}57$ & $5.8e{-14}$ \\\hline
\multirow{2}{*}{\texttt{ca2010}} & \multirow{2}{*}{$38$\%} & \multirow{2}{*}{$103$} & $10$ & $360$ & $3,600$ & $\phantom{0}34$ & $5.2e{-12}$ \\
 & & & $\phantom{0}1$ & $570$ & $\phantom{0,{}}570$ & $\phantom{0}52$ & $2.3e{-14}$ \\\hline
\multirow{2}{*}{\texttt{delaunay\_n20}} & \multirow{2}{*}{$\phantom{0}9$\%} & \multirow{2}{*}{$\phantom{0}35$} & $22$ & $150$ & $3,300$ & $\phantom{0}27$ & $1.8e{-13}$ \\
 & & & $\phantom{0}1$ & $630$ & $\phantom{0,{}}630$ & $\phantom{0}82$ & $9.8e{-14}$ \\\hline
\multirow{2}{*}{\texttt{rgg\_n\_2\_20\_s0}} & \multirow{2}{*}{$15$\%} & \multirow{2}{*}{$\phantom{0}24$} & $17$ & $120$ & $2,040$ & $\phantom{0}26$ & $3.2e{-10}$ \\
 & & & $\phantom{0}1$ & $420$ & $\phantom{0,{}}420$ & $\phantom{0}44$ & $4.1e{-8}$ \\\hline
\end{tabular}

==> graph_table2.tex <==
\begin{tabular}{lcccc}
\hline
\multirow{2}{*}{Matrix} & \multirow{2}{*}{$m$} & \multirow{2}{*}{iters} & \multirow{2}{*}{ORTH}& \multirow{2}{*}{MV} \\
 & & & & \\\hline
\hline
\multirow{2}{*}{\texttt{caidaRouterLevel}} & $10$ & $570$ & $47$\% & $15$\%\\
  & $\phantom{0}1$ & $780$ & $38$\% & $\phantom{0}1$\%\\\hline
\multirow{2}{*}{\texttt{mn2010}} & $10$ & $360$ & $52$\% & $12$\%\\
  & $\phantom{0}1$ & $510$ & $54$\% & $\phantom{0}1$\%\\\hline
\multirow{2}{*}{\texttt{coPapersDBLP}} & $\phantom{0}9$ & $360$ & $32$\% & $41$\%\\
  & $\phantom{0}1$ & $630$ & $56$\% & $\phantom{0}6$\%\\\hline
\multirow{2}{*}{\texttt{ca2010}} & $10$ & $360$ & $54$\% & $12$\%\\
  & $\phantom{0}1$ & $570$ & $68$\% & $\phantom{0}1$\%\\\hline
\multirow{2}{*}{\texttt{delaunay\_n20}} & $22$ & $150$ & $33$\% & $19$\%\\
  & $\phantom{0}1$ & $630$ & $69$\% & $\phantom{0}1$\%\\\hline
\multirow{2}{*}{\texttt{rgg\_n\_2\_20\_s0}} & $17$ & $120$ & $26$\% & $19$\%\\
  & $\phantom{0}1$ & $420$ & $72$\% & $\phantom{0}2$\%\\\hline
\end{tabular}

==> groundstates_table.tex <==
\begin{tabular}{l|c|c|c|c|c|c}
\hline
\multirow{2}{*}{Matrix} & \multirow{2}{*}{$\delta$} & \multirow{2}{*}{iters} & \multirow{2}{*}{MV} & \multirow{2}{*}{Time(s)} & \multirow{2}{*}{$nev$} & \multirow{2}{*}{residual} \\
 & & & & & & \\\hline
\hline
 & $\phantom{0}50$ & $\phantom{0}3$ & $\phantom{0}13,500$ & $\phantom{0}18$ & $103$ & $2.8e{-13}$ \\
\verb|Ge87H76| & $100$ & $\phantom{0}4$ & $\phantom{0}36,000$ & $\phantom{0}40$ & $185$ & $2.0e{-12}$ \\
 & $\phantom{0}92$ & $\phantom{0}4$ & $\phantom{0}33,120$ & $\phantom{0}38$ & $103$ & $1.6e{-12}$ \\\hline
 & $\phantom{0}50$ & $\phantom{0}3$ & $\phantom{0}13,500$ & $\phantom{0}19$ & $117$ & $2.9e{-13}$ \\
\verb|Ge99H100| & $100$ & $\phantom{0}3$ & $\phantom{0}27,000$ & $\phantom{0}32$ & $107$ & $8.9e{-13}$ \\
 & $\phantom{0}92$ & $\phantom{0}3$ & $\phantom{0}24,840$ & $\phantom{0}28$ & $110$ & $7.2e{-13}$ \\\hline
 & $\phantom{0}50$ & $\phantom{0}3$ & $\phantom{0}13,500$ & $\phantom{0}33$ & $128$ & $1.9e{-13}$ \\
\verb|Si41Ge41H72| & $100$ & $\phantom{0}3$ & $\phantom{0}27,000$ & $\phantom{0}56$ & $116$ & $1.2e{-12}$ \\
 & $118$ & $\phantom{0}4$ & $\phantom{0}42,480$ & $\phantom{0}86$ & $200$ & $3.6e{-12}$ \\\hline
 & $\phantom{0}50$ & $\phantom{0}3$ & $\phantom{0}13,500$ & $\phantom{0}32$ & $108$ & $1.7e{-13}$ \\
\verb|Si87H76| & $100$ & $\phantom{0}5$ & $\phantom{0}45,000$ & $\phantom{0}93$ & $219$ & $4.5e{-12}$ \\
 & $134$ & $\phantom{0}4$ & $\phantom{0}48,240$ & $\phantom{0}94$ & $119$ & $4.5e{-12}$ \\\hline
 & $\phantom{0}50$ & $13$ & $\phantom{0}58,500$ & $215$ & $115$ & $7.4e{-16}$ \\
\verb|Ga41As41H72| & $100$ & $\phantom{0}9$ & $\phantom{0}81,000$ & $223$ & $145$ & $4.7e{-16}$ \\
 & $141$ & $\phantom{0}8$ & $101,520$ & $262$ & $105$ & $4.6e{-16}$ \\\hline
 & $200$ & $\phantom{0}5$ & $\phantom{0}90,000$ & $187$ & $178$ & $1.3e{-11}$ \\
\verb|Laplacian| & $300$ & $\phantom{0}4$ & $108,000$ & $199$ & $121$ & $1.8e{-11}$ \\
 & $273$ & $\phantom{0}4$ & $\phantom{0}98,280$ & $187$ & $139$ & $1.9e{-11}$ \\\hline
 & $\phantom{0}50$ & $\phantom{0}4$ & $\phantom{0}18,000$ & $\phantom{0}15$ & $134$ & $5.0e{-15}$ \\
\verb|Qdot3| & $100$ & $\phantom{0}6$ & $\phantom{0}54,000$ & $\phantom{0}31$ & $108$ & $1.3e{-13}$ \\
 & $118$ & $\phantom{0}5$ & $\phantom{0}53,100$ & $\phantom{0}26$ & $209$ & $2.5e{-13}$ \\\hline
\end{tabular}
